Classical and Quantum algorithms for generic Syndrome Decoding problems and applications to the Lee metric

The security of code-based cryptography usually relies on the hardness of the syndrome decoding (SD) problem for the Hamming weight. The best generic algorithms are all improvements of an old algorithm by Prange, and they are known under the name of Information Set Decoding (ISD) algorithms. This work aims to extend ISD algorithms' scope by changing the underlying weight function and alphabet size of SD. More precisely, we show how to use Wagner's algorithm in the ISD framework to solve SD for a wide range of weight functions. We also calculate the asymptotic complexities of ISD algorithms both in the classical and quantum case. We then apply our results to the Lee metric, which currently receives a significant amount of attention. By providing the parameters of SD for which decoding in the Lee weight seems to be the hardest, our study could have several applications for designing code-based cryptosystems and their security analysis, especially against quantum adversaries.

==> macro.tex <==
%Raccourcis
\let\ds\mathds

\usepackage{scalerel,stackengine}
\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern.1pt\mathchar"0362\kern.1pt}%
    {\rule{0ex}{\textheight}}%WIDTH-LIMITED CIRCUMFLEX
  }{\textheight}% 
}{2.4ex}}%
\stackon[-6.9pt]{#1}{\tmpbox}%
}
%Notations quantiques
%\newcommand{\norm}[1]{\left|\!\left| #1 \right|\!\right|}
\newcommand{\QFT}[1]{\reallywidehat{\ket{#1}}}

%Notations italiques
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cS}{\mathcal{S}}

%Notations double barre
\newcommand{\C}{\mathbb{C}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zq}{\Z_q}
\newcommand{\Fq}{\F_q}

%Intervalle
\newcommand{\interv}{[\![-\frac{q-1}{2},\frac{q-1}{2}]\!]}
\newcommand{\interval}[2]{\left[\!\!\left[#1,#2\right]\!\!\right]}
%Code
\newcommand{\CC}{\ensuremath{\mathscr{C}}}

\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\algo}[1]{\mathcal{#1}}
\newcommand{\set}[1]{\mathcal{#1}}

%lettres calligraphiques
\newcommand{\Ac}{{\mathcal A}}
\newcommand{\Bc}{{\mathcal B}}
\newcommand{\Dc}{{\pazocal D}}
\newcommand{\Ec}{{\pazocal E}}
\newcommand{\Gc}{{\mathcal G}}
\newcommand{\Hc}{{\mathcal H}}
\newcommand{\Pc}{{\mathcal P}}
\newcommand{\Sc}{{\mathcal S}}
\newcommand{\Tc}{{\mathcal T}}
\newcommand{\Uc}{{\mathcal U}}
\newcommand{\Vc}{{\mathcal V}}
\newcommand{\Xc}{{\mathcal X}}

%Vecteurs
\newcommand{\av}{\vec{a}}
\newcommand{\bv}{\vec{b}}
\newcommand{\cv}{\vec{c}}
\renewcommand{\dv}{\vec{d}}
\renewcommand{\ev}{\vec{e}}
\newcommand{\sv}{\vec{s}}
\newcommand{\tv}{\vec{t}}
\newcommand{\uv}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\wv}{\vec{w}}
\newcommand{\xv}{\vec{x}}
\newcommand{\yv}{\vec{y}}
\newcommand{\zv}{\vec{z}}
\newcommand{\zero}[1]{\vec{0}_{#1}}
\newcommand{\un}{\vec{1}}
\newcommand{\und}{\mathds{1}}

%Matrices
\newcommand{\Am}{\vec{A}}
\newcommand{\Bm}{\vec{B}}
\newcommand{\Cm}{\vec{C}}
\newcommand{\Dm}{\vec{D}}
\newcommand{\Em}{\vec{E}}
\newcommand{\Fm}{\vec{F}}
\newcommand{\Gm}{\vec{G}}
\newcommand{\Hm}{\vec{H}}
\newcommand{\Mm}{\vec{M}}
\newcommand{\Nm}{\vec{N}}
\newcommand{\Pm}{\vec{P}}
\newcommand{\Rm}{\vec{R}}
\newcommand{\Sm}{\vec{S}}
\newcommand{\Tm}{\vec{T}}
\newcommand{\Um}{\vec{U}}
\newcommand{\Xm}{\vec{X}}
\newcommand{\Ym}{\vec{Y}}
\newcommand{\Zm}{\vec{Z}}
\newcommand{\Had}[2]{\mat{H}_{#1,#2}} % Hadamard gate
\newcommand{\Id}{\vec{Id}}

%Probabilites
\newcommand{\esp}{\mathbb{E}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\prob}{\pi_{\ev}}
\newcommand{\probdual}{\hat{\pi}_{\cv^\perp}}

%Sommes
\newcommand{\subV}{\substack{V \le \Fq^m \\ \dim V = t}}
\newcommand{\sumV}{\sum_{\subV}}
\newcommand{\sumW}{\sum_{\substack{W \le \Fq^m \\ \dim W = t \\ W \neq V}}}
\newcommand{\subyt}{\substack{\vec{y} \in \Fq^n \\ \wt{y} = t}}
\newcommand{\sumyt}{\sum_{\subyt}}

\newcommand{\sumFq}[1]{\sum_{#1 \in \Fq^\ast}}
\newcommand{\sumFqn}[1]{\sum_{\vec{#1} \in \Fq^n}}
\newcommand{\sumcode}{\sum_{\cv \in \CC}}
\newcommand{\sumdual}{\sum_{\cv^\perp \in \CC^\perp}}

%Valeurs entieres superieure et inferieure
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

%Coefficients gaussiens
\newcommand{\gauss}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}

%Produit scalaire
\newcommand{\innerprod}[2]{\vec{#1} \cdot \vec{#2}}

%Poids et distances
\newcommand\wt[1]{\abs{\vec{#1}}}
\newcommand{\dr}{d_{\textup{rank}}}
\newcommand\wtr[1]{\abs{\vec{#1}}_{\textup{rank}}}
\newcommand\wth[1]{\abs{\vec{#1}}_{\textup{Ham}}}
\newcommand\wtl[1]{\abs{\vec{#1}}_{\textup{Lee}}}
\newcommand\dl{d_{\textup{Lee}}}
\newcommand{\weasy}{w_{\textup{easy}}}
\newcommand{\omeasy}{\omega_{\textup{easy}}}

%Distances
\newcommand{\dgv}{d_{\textup{GV}}}
\newcommand{\drgv}{\tau_{\textup{GV}}}
\newcommand{\dmin}{d_{\textup{min}}}
\newcommand{\dtr}{D_{\textup{tr}}}
\newcommand{\dstat}{D_{\textup{stat}}}

%etats intermediaires de la reduction
\newcommand{\psiA}{\ket{\psi_{\Ac}}}
\newcommand{\psiAQFT}{\ket{\psi_{\Ac}^{\textup{QFT}}}}
\newcommand{\psiideal}{\ket{\psi_{\text{ideal}}}}
\newcommand{\psiidealQFT}{\ket{\psi_{\text{ideal}}^{\textup{QFT}}}}
\newcommand{\psiAs}{\psi_{\Ac}}
\newcommand{\psiideals}{\psi_{\text{ideal}}}

%Trace
\newcommand{\Trac}[2]{\textup{Tr}_{#1 / #2}}

%operateurs mathematiques
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
%\DeclareMathOperator*{\rank}{Rank}

% \OO{ } : grand O de { }
\newcommand{\OOtsp}[1]{O(#1)} % OO textstyle parentheses --> to be preferred to avoid vertical space ugliness
\newcommand{\Thtsp}[1]{\Theta(#1)} % Theta textstyle parentheses --> to be preferred to avoid vertical space ugliness
\newcommand{\OO}[1]{O\left( #1 \right)}
\newcommand{\Th}[1]{\Theta\left( #1 \right)}
\newcommand{\Tht}[1]{\tilde{\Theta}\left( #1 \right)}
\newcommand{\OOt}[1]{\tilde{O}\left( #1 \right)}
\newcommand{\Om}[1]{\Omega \left( #1 \right)}
\newcommand{\Omt}[1]{\tilde{\Omega} \left( #1 \right)}

%Transposition
\makeatletter
\newcommand*{\transp}{{\mathpalette\@transpose{}}}
\newcommand*{\@transpose}[2]{\raisebox{\depth}{$\m@th#1\intercal$}}
\makeatother
\newcommand{\transpose}[1]{{#1}^{\transp}}
\newcommand{\tran}[1]{\transpose{#1}}

%Def equal
\newcommand*{\eqdef}{\stackrel{\text{def}}{=}}

%Probleme 
\newcommand{\sdecP}{\textup{$\mathsf{SDP}$}}
\newcommand{\SDP}{\sdecP}
\newcommand{\scodeP}{\textup{$\mathsf{SCP}$}}
\newcommand{\SCP}{\scodeP}
%JP: je mets des macros supplémentaires, je ne comprends pas la logique de ces abréviations et je suis incapable de m'en souvenir quand je les ecris.

%Environnement 
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{notation}{Notation}
\newtheorem{fact}{Fact}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{assumption}{Assumption}
\newtheorem{rthumb}{Rule of thumb}

%Style
\renewcommand{\thefootnote}{\texttt{(\arabic{footnote})}} % Numéros des notes de bas de page plus lisibles
\renewcommand{\baselinestretch}{1.1} % Espacement des lignes
\sloppy % Espacement des mots plutôt que césure
\setlength{\parindent}{0pt} % Empêcher les alinéas
\setlength{\parskip}{3pt} % Espacement des paragraphes
\renewcommand*\thesection{\arabic{section}}

%commandes pour les commentaires
\newcommand{\jp}[1]{{\textcolor{red}{JP: #1}}}
\newcommand{\andre}[1]{{\color{blue} André: #1 \color{black}}}
\newcommand{\simona}[1]{{\color{blue} Simona: #1 \color{black}}}
\newcommand{\toto}[1]{{\color{green} Toto: #1 \color{black}}}

%André
\newcommand{\zo}{\{0,1\}}

%<<<<<<< HEAD
%\newtheorem{assumption}{Assumption}
%=======
%>>>>>>> 290ea4bbd9c9ade0af00bc789a69c3012d760d39
%<<<<<<< HEAD
%
%=======
%>>>>>>> 7be7f12c04722a9a453421ba8af42f07d1355d5d

% FOR HAVING SEVERAL KEYS FOR THE SAME BIBLIOGRAPHIC ENTRY

 \makeatletter
% \bibalias{<alias>}{<source>} makes \cite{<alias>} equivalent to \cite{<source>}
\newcommand\bibalias[2]{%
  \@namedef{bibali@#1}{#2}%
}

\newtoks\biba@toks
\newcommand\acite[2][]{%
  \biba@toks{\cite#1}%
  \def\biba@comma{}%
  \def\biba@all{}%
  \@for\biba@one:=#2\do{%
    \@ifundefined{bibali@\biba@one}{%
      \edef\biba@all{\biba@all\biba@comma\biba@one}%
    }{%
      \PackageInfo{bibalias}{%
        Replacing citation `\biba@one' with `\@nameuse{bibali@\biba@one}'
      }%
      \edef\biba@all{\biba@all\biba@comma\@nameuse{bibali@\biba@one}}%
    }%
    \def\biba@comma{,}%
  }%
  \edef\biba@tmp{\the\biba@toks{\biba@all}}%
  \biba@tmp
}
\makeatother

\bibalias{Ouroboros-R}{AABBBDGHZ17}
\bibalias{RQC}{AABBBDGZ17}
\bibalias{RQC2}{AABBBDGZCH19}
\bibalias{ROLLO}{ABDGHRTZABBBO19}
\bibalias{LAKE}{ABDGHRTZ17}
\bibalias{LOCKER}{ABDGHRTZ17a}
\bibalias{RankSign}{AGHRZ17}

